Model-Free Feedback Constrained Optimization Via Projected Primal-Dual Zeroth-Order Dynamics

In this paper, we propose a model-free feedback solution method to solve generic constrained optimization problems, without knowing the specific formulations of the objective and constraint functions. This solution method is termed projected primal-dual zeroth-order dynamics (P-PDZD) and is developed based on projected primal-dual gradient dynamics and extremum seeking control. In particular, the P-PDZD method can be interpreted as a model-free controller that autonomously drives an unknown system to the solution of the optimization problem using only output feedback. The P-PDZD can properly handle both the hard and asymptotic constraints, and we develop the decentralized version of P-PDZD when applied to multi-agent systems. Moreover, we prove that the P-PDZD achieves semi-global practical asymptotic stability and structural robustness. We then apply the decentralized P-PDZD to the optimal voltage control problem in power distribution systems with square probing signals, and the simulation results verified the optimality, robustness, and adaptivity of the P-PDZD method.

==> Algorithm.tex <==


\section{Exponential Stability and Tracking Performance} \label{sec:algorithm}
%












\subsection{Regularization and Exponential Stability}



\begin{assumption}\label{ass:strongconvex}
The objective function $f(\bx)$ in \eqref{eq:general:obj} is twice differentiable, $\mu$-strongly convex and $\ell$-smooth with $0<\mu\leq \ell$, i.e., for all $\bx_1,\bx_2\in\R^d$, we have
\begin{align}
\begin{split}
    \mu ||\bx_1-\bx_2||^2\leq (\nabla f(\bx_1) - \nabla f(\bx_2))^\top (&\bx_1-\bx_2)\\
      \leq \ell ||&\bx_1-\bx_2||^2.
\end{split}
\end{align}
\end{assumption}


Consider the regularized  saddle point problem \eqref{eq:saddle:regu}:
\begin{align}\label{eq:saddle:regu}
   \max_{\bla\in \R_+^m} \min_{\bx\in\mathcal{X}}\   L_{\delta} (\bx,\bla) := L(\bx,\bla) - \frac{\delta}{2}||\bla||^2,
\end{align}
where $L_\delta(\bx,\bla)$ is the regularized Lagrangian function, and
$\delta>0$ is the regularization parameter. 
As a result, $L_{\delta}(\bx,\bla)$ is strongly concave in the dual variable $\bla$ and strongly convex in the primal variable $\bx$ under Assumption \ref{ass:con_sm} and \ref{ass:strongconvex}\footnote{When
the objective function $f(\bx)$ itself is not strongly convex in $\bx$, i.e., Assumption \ref{ass:strongconvex} does not hold, the similar regularization method can be used by adding the term $\frac{\delta_x}{2} ||\bx||^2$ to the regularized Lagrangian function to impose strong convexity on $\bx$.}, which indicates that the optimal solution of \eqref{eq:saddle:regu} is unique.
However, due to the regularization term $\frac{\delta}{2}||\bla||^2$, the optimal solution of \eqref{eq:saddle:regu} is different from that of the original saddle point problem \eqref{eq:saddle}. Let $\bz^*:=[\bx^*;\bla^*]$ and $\bz_\delta^*:=[\bx_\delta^*;\bla_\delta^*]$  be the optimal solution of \eqref{eq:saddle} and \eqref{eq:saddle:regu}, respectively. The following proposition provides a theoretic bound for  the difference.

\begin{proposition}
Error of optimal solution, blabla...
\end{proposition}

The regularized projected primal-dual gradient dynamics (\textbf{R-P-PDGD})   are given by
\begin{align}  \label{eq:rppdgd:la}
\begin{split}
    &  \text{Equation }\eqref{eq:ppdgd:x}\\
  &     \dot{\lambda}_j = \mathrm{Proj}_{\R_+}\big[ \lambda_j + \alpha_\lambda\, (g_j(\bx)-\delta \lambda_j)
     \big] -\lambda_j,\   j\in[m].  
\end{split}
\end{align}



\begin{theorem} \label{thm:exponential}
(Global Exponential Stability.) %Let $\mathbf{z}_1:=[\bx^\top,\bla^\top]$ and $\mathbf{z}_1^*:=[\bx^{*\top},\bla^{*\top}]$, were $\bx^*$ is an optimal solution of the OVC problem (\ref{eq:ovc}). 
Under  Assumption \ref{ass:con_sm}, \ref{ass:finite} and \ref{ass:strongconvex}, 
with initial condition $\bz(0)\in \sZ$, the trajectory $\bz(t)$ of the P-PDGD (\ref{eq:ppdgd}) will stay within $\sZ$ for all $t\geq 0$ and globally exponentially converge to an optimal solution $\bz^*:=[\bx^*;\bla^*]$ of the saddle point problem (\ref{eq:saddle}). 
\end{theorem}

Similarly,
the regularized zeroth-order feedback dynamics (\textbf{R-ZOFD}) are formulated as    
\begin{align}  \label{eq:rppdgd:la}
\begin{split}
  &  \text{Equations }  \eqref{eq:es:ppdgd:x}, \eqref{eq:es:ppdgd:psi}- \eqref{eq:es:ppdgd:mu},\\
    & \dot{\lambda}_j = \mathrm{Proj}_{\R_+}\big[ \lambda_j + \alpha_\lambda\, (\mu_j-\delta \lambda_j)
     \big] -\lambda_j,\   j\in[m].
\end{split}
\end{align}

\begin{theorem} \label{thm:sgpes}
(Semi-Global Practical Exponential Stability.) ...
\end{theorem}

\subsection{Tracking Performance } \label{sec:track}


\begin{assumption}
\begin{align}
    ||\frac{d\bz^*(t)}{dt}||\leq \rho
\end{align}
\end{assumption}




==> Distributed.tex <==


\section{Application to Multi-Agent Systems}
\label{sec:distributed}

This section studies the multi-agent variant of problem \eqref{eq:gen} and develops distributed model-free solution algorithms. bla bla bla.... abstract of this section.

\subsection{Multi-Agent Problem  Setting}
 

 
For Problem Setting 1, the proposed ES-CP-PDGD \eqref{eq:es:cppdgd} and ES-DP-PDGD \eqref{eq:es:dppdgd} can be directly implemented in a distributed fashion. Specifically, each agent $i\in[N]$ implements its own action $\hat{\bx}_i(t):= \bx_i(t) + a\sin(\bom_i t)$,  receives the system feedback $f(\hat{\bx}(t))$ and $\bg(\hat{\bx}(t))$, and then updates  actions according to its own part of dynamics in \eqref{eq:es:cppdgd} or 
\eqref{eq:es:dppdgd}. The dynamics of $\bx$ in \eqref{eq:es:cppdgd:x} and \eqref{eq:es:dppdgd:x} is decomposable over agents, so that each agent $i$ can implement it independently  with the projection to its own feasible set $\sX_i$.   
 
\begin{problem}
\normalfont There is a directed communication graph $G([N],\sE)$ over the agents, where $[N]$ is the node set and $\sE\subseteq [N]\times [N]$ is the edge set. Node $i\in [N]$ corresponds to agent $i$, and $ij\in \sE$   means that agent $j$ can send information to its neighbor agent $i$.  The agents aim to cooperatively find an optimal solution that solves the  problem  \eqref{eq:dist}:
\begin{subequations} \label{eq:dist} 
\begin{alignat}{2}
      \text{Obj.} \ \, &   \min_{\bx}\, f(\bx)= \sum_{i=1}^N  && f_i(\bx) \label{eq:dist:obj} \\
    \text{s.t.} \ \  & \, \bx_i\in \sX_i, &&  i=1,\cdots,N         \\
    & \, \bg_i(\bx) \leq 0, && i=1,\cdots, N,\label{eq:dist:con}
\end{alignat}
\end{subequations}
where $f_i:\R^n\to\R$ is the local cost function  and function vector $\bg_i:\R^n\to \R^{m_i}$ depicts the local  constraints for agent $i$ with $\sum_{i=1}^N m_i=m$. Functions $f_i$ and $\bg_i$ depend on the joint action profile $\bx$. Each agent $i\in[N]$  knows its own feasible set $\sX_i$ and can only access the function evaluations of its local functions $f_i$ and $\bg_i$. Besides, agent $j$ can send information to agent $i$ if $ij\in\sE$ and receive information from agent $k$ if $jk\in\sE$.
\qed

\end{problem}
 
The problem \eqref{eq:dist} is  a special case of  \eqref{eq:gen}, and it is 
motivated by a variety of multi-agent networked systems, such as power grids [xx], transportation systems [xx], communication networks [xx], etc. 


In the follows, we focus on Problem Setting 2 and develop  distributed model-free feedback algorithms to solve it based on the ES-CP-PDGD \eqref{eq:es:cppdgd} and ES-DP-PDGD \eqref{eq:es:dppdgd} algorithms.

\subsection{Distributed Model-Free Feedback Algorithms}

To solve the problem \eqref{eq:dist}, similarly, we introduce the dual variable $\bla_i\in\R_+^{m_i}$ for each inequality constraint in \eqref{eq:dist:con} and formulate the saddle point problem of \eqref{eq:dist} as 
\begin{align} 
     \max_{\bla\in \R_+^m}\,  \min_{\bx_i\in\mathcal{X}_i}\, L(\bx,\bla):=\sum_{i=1}^N f_i(\bx)+\sum_{i=1}^N \bla_i^\top \bg_i(\bx).
\end{align}
%
However,
the ES-CP-PDGD \eqref{eq:es:cppdgd} and ES-DP-PDGD \eqref{eq:es:dppdgd} can not be implemented distributedly in this case, since the update of $\bpsi$ in \eqref{eq:es:cppdgd:psi} 
needs 
the function evaluations of $\{f_i,\bg_i\}_{i\in[N]}$ over all agents, namely the global term $\sum_{i=1}^N(f_i+ \bla_i^\top \bg_i)$.
Fortunately, this global term is a summation of local signals  over all agents, thus
the  dynamic  average  consensus  methods  \cite{kia2019tutorial} can be employed to address this issue by leveraging  the local communications  with   neighbors.

Accordingly, based on the ES-CP-PDGD \eqref{eq:es:cppdgd}, we develop the distributed ES-CP-PDGD (\textbf{D-ES-CP-PDGD}) as \eqref{eq:d:cp}:
\begin{subequations} \label{eq:d:cp}
\begin{align}
        \dot{\bx}_i &= k_x\Big[\mathrm{Proj}_{\hat{\sX}_i}\big( \bx_i - \alpha_x \bpsi_i \big) -\bx_i\Big] \label{eq:d:cp:x} 
  \\
   \dot{\bla}_i & = k_{\lambda}\Big[\mathrm{Proj}_{\R_+^{m_i}}\big( \bla_i + \alpha_\lambda \bmu_i
     \big) -\bla_i\Big] \label{eq:d:cp:la}\\
     \dot{\bpsi}_i& = \,\frac{1}{\epsilon}\, \Big[ \!-\!\bpsi_i + \frac{2N}{a} y_i(t)\sin(\bom_i t)    \Big]  \label{eq:d:cp:psi}\\ 
 \dot{\bmu}_i &= \,\frac{1}{\epsilon}\,\Big[ -\bmu_i + \bg_i (\hat{\bx}(t)) \Big] \label{eq:d:cp:mu}\\
 \dot{p}_i &=  \frac{1}{\epsilon_p}\cdot\sum_{ij\in \mathcal{E}} a_{ij}(y_i(t) - y_j(t))\label{eq:d:cp:p}\\
 y_i(t)&= f_i(\hat{\bx}(t)) + \bla_i(t)^\top \bg_i(\hat{\bx}(t)) - p_i(t), \label{eq:d:cp:y}
\end{align}
\end{subequations}
where $\epsilon_p$ is a small positive parameter, and $a_{ij}$ is the associated element in the  weighted adjacency matrix $A\in \R^{N\times N}$. $a_{ij}>0$ if $ij\in\sE$, and $a_{ij}=0$ otherwise. Moreover, the initialization condition $\sum_{i=1}^Np_i(t_0) =0$ should be enforced to ensure zero steady-state tracking error of the consensus algorithm. 
This condition can be easily satisfied if each agent $i$ sets $p_i(t_0) =0 $ as $p_i$ is an internal intermediate variable. In addition,
some advanced dynamic average consensus algorithms, e.g.,  \cite{freeman2006stability}, can also be adopted to circumvent this initialization requirement.

Equation \eqref{eq:d:cp:p} is the consensus update using local communications.
Intuitively,
$ y_i$ defined in \eqref{eq:d:cp:y} is interpreted as agent $i$'s local tracking signal of the global average term $\frac{1}{N}\sum_{i=1}^N(f_i+ \bla_i^\top \bg_i)$. Besides, the introduction of variable $p_i$ is  a commonly-used change of  variable \cite{kia2019tutorial} to avoid additional time derivative terms in the dynamics \eqref{eq:d:cp}.

Similarly, based on the ES-DP-PDGD \eqref{eq:es:dppdgd}, we develop the distributed ES-DP-PDGD (\textbf{D-ES-DP-PDGD}) as \eqref{eq:d:dp}:
\begin{subequations} \label{eq:d:dp}
\begin{align}
      &   \dot{\bx}_i  = k_x\cdot\mathrm{Proj}_{T_{\hat{\sX}_i}(\bx)}\big( - \bpsi_i  \big)  \label{eq:d:dp:x}
  \\
     &\dot{\bla}_i =k_\lambda\cdot \mathrm{Proj}_{T_{\R_+^{m_i}}(\bla_i)}\big(   \bmu_i
     \big) \label{eq:d:dp:la}
     \\
    & \text{Equations \eqref{eq:d:cp:psi}-\eqref{eq:d:cp:y}}.
\end{align}
\end{subequations}


\subsection{Analysis of D-ES-CP-PDGD and D-ES-DP-PDGD}

We make the  following standard assumption on the communication graph $G$ and the  weighted adjacency matrix $A$.

 \begin{assumption}\label{ass:graph}
 The weighted directed graph $G([N],\mathcal{E},A)$ is weight-balanced and strongly connected.
 \end{assumption}


========================================











\begin{example}
\normalfont (Optimal Power Flow). Consider a power network with the bus set $\mathcal{V}$, the line set $\mathcal{E}$, and the generator  set $\mathcal{G}$. For each generator (agent) $i\in \mathcal{G}$, the action is the active and reactive power injection, i.e., $\bx_i:=[p_i;q_i]$,
and $\sX_i$ represents the associated power capacity constraints given by
\begin{align}
    \sX_i:= \{ \bx_i: 0\leq p_i \leq \bar{p}_i,\, p_i^2+q_i^2\leq \bar{s}_i^2\}, 
\end{align}
where $\bar{p}_i$ is the maximal power generation limit  and $\bar{s}_i$ denotes the apparent power capacity of generator $i$.




Here, $c_0(\bx)$ is the system operation cost, e.g., network loss, and $c_i(\bx_i)$ is the generation cost of generator $i$. 
$P_j(\bx)$ denotes the power flow of line $j\in\mathcal{E}$ , and $\bar{P}_{j}$ and $\underline{P}_{j}$ denote the upper and lower limits respectively. $v_k(\bx)$ is the voltage magnitude of bus $k\in\mathcal{V}$ that should be within the interval $[\underline{v}_k,\bar{v}_k]$. The functions $c_0(\bx)$, $(P_j(\bx))_{j\in\mathcal{E}}$, and $(v_k(\bx))_{k\in \mathcal{V}}$ capture the power flow equations, network topology, network parameters, loads and other uncontrollable power injections, etc. It is generally difficult to estimate these functions accurately  for large-scale power systems, and the system is time-varying due to changing operation conditions, volatile renewable generation, natural disasters, etc. 




\end{example}

\begin{example}
\normalfont (Communication networks)
\end{example}










